TradAO: A Visual Analytics System for Trading Algorithm Optimization

With the wide applications of algorithmic trading, it has become critical for traders to build a winning trading algorithm to beat the market. However, due to the lack of efficient tools, traders mainly rely on their memory to manually compare the algorithm instances of a trading algorithm and further select the best trading algorithm instance for the real trading deployment. We work closely with industry practitioners to discover and consolidate user requirements and develop an interactive visual analytics system for trading algorithm optimization. Structured expert interviews are conducted to evaluateTradAOand a representative case study is documented for illustrating the system effectiveness. To the best of our knowledge, previous financial data visual analyses have mainly aimed to assist investment managers in investment portfolio analysis but have neglected the need of traders in developing trading algorithms for portfolio execution.TradAOis the first visual analytics system that assists users in comprehensively exploring the performances of a trading algorithm with different parameter settings.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> src/background.tex <==
\section{Background}
\subsection{Data Overview}
The data used in our visualization system is based on a set of backtesting records, provided by ALGOGENE platform\footnote{\href{https://algogene.com/}{https://algogene.com/}}. There are in total xxxxxxxxx backtesting records of various trading strategies. Each backtesting record represents a dynamic portfolio driven by an underlying trading strategy. 

The portfolio of a trading strategy could be constructed from multiple financial instruments ranging from Currency Pairs, Metals, Commodities, Interest Rate Future to Equity Index CFDs, with their corresponding historical dataset over a time horizon from 2010 to 2019. Each financial instrument contains three tick level information attributes, including Price, Volume, and Order Book details on Bid and Ask direction. Depending on its market liquidity, each financial instrument has about 100 thousands to over 1 million of tick records in a particular trading month. At each tick moment, a trading portfolio consisting a combination of cash and financial instruments with corresponding portfolio weights, varies in performance over time. 

% \subsection{Data Model}
\subsection{Trading Strategy}
Our visualization system could be generally applicable to all different scenarios of trading strategies and market regimes. In this paper, three widely used trading strategies are particularly selected for demonstration, namely Moving Average, Pair Trading, and Regression Model. These three trading strategies are relatively less complexed in terms of the used amount of parameters.

\paragraph{Moving Average}
Moving Average Model, a subclass of ARIMA model, usually applies to univariate time series for studying the relationship between a variable and its lagged terms~\cite{background_f}. Traders base on this model to analyze the seasonal effect of financial instruments, where the underlying time series appear to fluctuate at a regular interval~\cite{background_f}.

\paragraph{Pair Trading}
Pair Trading is a market neutral strategy that opens long and short position for 2 securities simultaneously to capture the price differential. A trading pair could be dynamically constructed from all the available financial instruments over  different trading horizons. On a particular trading day with N available instruments, it could constitute to a maximum of $N(N-1)/2$ possible trading pair combinations. Traders adopt various methodologies for the price distance measurement and trading pair identification and selection. 

\paragraph{Regression Model}
A Multiple Linear Regression Model is used for modelling a multi-variate time series ~\cite{background_g}. The price or return of a particular financial instrument could be explained by certain factors, which could be economic statistics, news sentiment indicators, or price and volume information of other financial instruments. 

% \subsubsection{Trading Parameter Correlation}
% Depending on the strategy complexity, algorithmic trading strategies consist of uneven number of trading parameters which could ranging from tens to hundreds, or even more. These parameters could either be static or dynamically changing throughout the trading horizon. For such a large parameter set, traders might then encounter the problems of (a) introducing a relatively more parameters compared to sampling size; (b) the similarity of trading parameters cannot be compared easily due to a non-linear scale of combinations $O(N^2)$. The trading parameter set should neither be too small for practical use, nor too large for potential overfitting or runtime inefficiency. To address the problem, we proposed a Filtered Sliding-Window Correlation mechanism in the Correlation View.

% At the initial system loading, only the recent one year of data series are pull to a data storage list. The window frame can subsequently be adjusted by user with extending the storage list for additional data. We then conduct a pre-process screening to filter out time series that are constant over the selected horizon which can effectively reduce majority of data series that is static in nature. In consideration of computational efficiency, the correlation series for the remaining trading parameter set are calculated using an iterative method as below:

% Denote $X_t$,$Y_t$ be the trading parameter value of any two arbitrary series at a specific time $t$. Suppose $0\leq t\leq t+h \leq T$, according to the definition of Pearson Correlation, 

% Now, we define 

% Thus, the correlation series can be deduced iteratively. 

% In the Correlation View, h is default to be 20 days representing one trading month at initial system loading, in which the value could be dynamically adjusted subject to user preference. In terms of computational complexity, our iterative algorithm largely reduce the computational complexity from $O(Th)$ to a linear space of $O(T)$.

% \subsection{System Pipeline}
% The system is a front-to-back web application consisting of three modules: database module, data service module, and visualization module. The database module, which is based on a NoSQL Distributed File System provided by ALGOGENE, contains two collections of information. One group of information includes market data that are directly captured or aggregated from financial markets, such as tick level market transaction price-volume, aggregated OHLC candle bar, and metadata and contract specification of financial securities. Another group of information contains strategy data that are evaluated and calculated from ALGOGENE backtest engine, such as strategy performance statistics, profit-loss, portfolio positions and exposures, account balance and capital usage, as well as trading model variable list and training parameters value, in a daily basis. The data service module based on ALGOGENE rest API, which adopts a standard RESTful protocol, to provide a data transmission channel to interact with backend database, such as to query data, or to perform high level computations. 







==> src/discussion.tex <==
\section{Discussion}
The interview in the evaluation reveals the system’s usability. Positive feedbacks from domain expert interviewees reflect that the system succeeds in satisfying user requirements and facilitating their current workflow in building trading algorithms. To the best of our knowledge, TAOT is the first visualization system analyzing the trading algorithm development. This paper might serve as a good foundation and we plan to enhance our system’s functionality. The current system emphasizes on the single trading strategy discovery. A new function of cross-strategy comparison can further assist traders in deciding the weight of funding to be assigned over a portfolio of multiple trading strategies. In term of system interactions, common technical analysis indicators from industry practices can be inserted into the view of major market indices, so that manual errors in interpretation can be avoided.

However, our system still faces several limitations. One of the limitation is the scalability of the algorithm evolution view. When traders built and run the same trading strategy for considerable amounts of times, the design of tree diagram might encounter the challenge of  displaying all nodes in a reasonable scale. Displaying selected clusters after the overview could be an acceptable remedy, which is a trade-off between information density and information delivery. This challenge is possible yet uncommon, as traders tend to develop new trading strategies periodically due to the dynamics of financial markets. Another limitation is the subjectivity of the performance metric choices for evaluation in the algorithm evolution view. The current metrics are derived from our domain experts’ empirical knowledge. However, a better approach is to offer an option list for users to determine their own evaluation metrics. 

